Evaluating the Effect of Centralization on Routing Convergence on a Hybrid BGP-SDN Emulation Framework

A lot of applications depend on reliable and stable Internet connectivity. These characteristics are crucial for mission-critical services such as telemedical applications. An important factor that can affect connection availability is the convergence time of BGP, the de-facto inter-domain routing (IDR) protocol in the Internet. After a routing change, it may take several minutes until the network converges and BGP routing becomes stable again. Kotronis et al propose a novel Internet routing approach based on SDN principles that combines several Autonomous Systems (AS) into groups, called clusters, and introduces a logically centralized routing decision process for the cluster participants. One of the goals of this concept is to stabilize the IDR system and bring down its convergence time. However, testing whether such approaches can improve on BGP problems requires hybrid SDN and BGP experimentation tools that can emulate multiple ASes. Presently, there is a lack of an easy to use public tool for this purpose. This work fills this gap by building a suitable emulation framework and evaluating the effect that a proof-of-concept IDR controller has on IDR convergence time.

==> utils.tex <==
%%%
%%% Figure stuff
%%%
\renewcommand{\topfraction}{1}
\renewcommand{\dbltopfraction}{1}
\renewcommand{\floatpagefraction}{1}
\renewcommand{\dblfloatpagefraction}{1}
\renewcommand{\textfraction}{0}
%\renewcommand{\baselinestretch}{.985}

%%
%% General definitions one needs all the time
%%

\newcommand{\nibp}{\noindent\hspace{0.3em}\textbullet\hspace{0.7em}}

\newcommand{\xref}[1]{Section~\ref{#1}}
%\newcommand{\xref}[1]{\S\ref{#1}}
\newcommand{\cref}[1]{Chapter~\ref{#1}}
\newcommand{\pxref}[1]{(\xref{#1})}
\newcommand{\fref}[1]{Figure~\ref{#1}}
\newcommand{\tref}[1]{Table~\ref{#1}}
\newcommand{\see}[1]{~(see \xref{#1})}
\newcommand{\first}{\emph{(i)}~}
\newcommand{\second}{\emph{(ii)}~}
\newcommand{\third}{\emph{(iii)}~}
\newcommand{\fourth}{\emph{(iv)}~}
\newcommand{\fifth}{\emph{(v)}~}
\newcommand{\sixth}{\emph{(iv)}~}

\newcommand{\zb}{z.\,B. \@}

\newcommand{\ie}{i.e., \@}
\newcommand{\eg}{e.g., \@}
\newcommand{\etc}{etc., \@}
\newcommand{\Ie}{That is, \@}
\newcommand{\Eg}{For example, \@}
\newcommand{\cf}{cf. \@}
\newcommand{\Cf}{Cf. \@}

\newcommand{\etal}{et~al.\xspace}

\newcommand{\perc}{\,\%\xspace}
\newcommand{\pert}{\,\textperthousand\xspace}

\newcommand{\checked}{\ding{52}\xspace}
\newcommand{\unchecked}{\ding{56}\xspace}

\newcommand{\lstfun}[1]{function \lstinline[basicstyle=\normalsize]{#1}\xspace}
\newcommand{\lstfuns}[2]{functions \lstinline[basicstyle=\normalsize]{#1} and \lstinline[basicstyle=\normalsize]{#2}\xspace}

% "smallitemize"-environment like "itemize" but more dense
\newenvironment{smallitemize}{%
\begin{itemize}%
\setlength{\parsep}{0.3ex}%
%\setlength{\itemindent}{-3ex}%
\setlength{\leftmargin}{0.1pt}%
\setlength{\listparindent}{-8ex}%
\setlength{\itemsep}{0.2ex}%
\setlength{\topsep}{0ex}%
\setlength{\parskip}{0ex}%
\setlength{\partopsep}{0ex}%
}{%
\end{itemize}
}%

% "smallenumerate"-environment like "enumerate" but more dense
\newenvironment{smallenumerate}{%
\begin{enumerate}%
\setlength{\parsep}{0.3ex}%
%\setlength{\itemindent}{-3ex}%
\setlength{\leftmargin}{0.1pt}%
\setlength{\listparindent}{-8ex}%
\setlength{\itemsep}{0.2ex}%
\setlength{\topsep}{0ex}%
\setlength{\parskip}{0ex}%
\setlength{\partopsep}{0ex}%
}{%
\end{enumerate}
}%

\definecolor{darkgreen}{rgb}{0,0.5,0}
\definecolor{brown}{rgb}{0.7,0.3,0}
\definecolor{darkblue}{rgb}{0,0,0.5}
\newcommand{\todo}[1]{\textit{\textcolor{red}{TODO: #1}}}
%\newcommand{\bernhard}[1]{\textit{Bernhard: #1}}
\newcommand{\vassilis}[1]{\textit{\textcolor{brown}{#1---Vassilis.}}}
\newcommand{\fontas}[1]{\textit{\textcolor{darkblue}{#1---Fontas.}}}
\newcommand{\bernhard}[1]{\textit{\textcolor{darkgreen}{#1---Bernhard.}}}

%\renewcommand{\todo}[1]{}

% mark changed wording from first submission
\newcommand{\new}[1]{\textcolor{blue}{#1}}
\newcommand{\discuss}[1]{\textit{\textcolor{green}{Discuss: #1}}}

%\definecolor{mygrey}{rgb}{0.8,0.8,0.8}

\newcounter{fn1}
\setcounter{fn1}{1}
\newcounter{fn2}
\setcounter{fn2}{2}
\newcounter{fn3}
\setcounter{fn3}{3}
\newcounter{fn4}
\setcounter{fn4}{4}
\newcounter{fn5}
\setcounter{fn5}{5}
\newcommand{\fnsym}[1]{$^{\fnsymbol{#1}}$}

\newcommand{\minisec}[1]{\noindent\textbf{#1}:}

%%%
%%% Definitions specific to some papers
%%%

\newcommand{\libpcap}{\textsc{libpcap}\xspace}
\newcommand{\winpcap}{\textsc{winpcap}\xspace}
\newcommand{\libz}{\textsc{libz}\xspace}
\newcommand{\tcpdump}{\textsc{tcpdump}\xspace}
\newcommand{\snort}{\textsc{snort}\xspace}
\newcommand{\ipsumdump}{\textsc{ipsumdump}\xspace}
\newcommand{\wireshark}{\textsc{Wireshark}\xspace}
\newcommand{\bro}{\textsc{Bro}\xspace}
\newcommand{\spbc}{\textsc{spbc}\xspace}


\newcommand{\centralization}{Routing Centralization\xspace}
\newcommand{\raas}{Routing-as-a-Service\xspace}

